What Is Missing In Homophily? Disentangling Graph Homophily For Graph Neural Networks

Graph homophily refers to the phenomenon that connected nodes tend to share similar characteristics. Understanding this concept and its related metrics is crucial for designing effective Graph Neural Networks (GNNs). The most widely used homophily metrics, such as edge or node homophily, quantify such "similarity" as label consistency across the graph topology. These metrics are believed to be able to reflect the performance of GNNs, especially on node-level tasks. However, many recent studies have empirically demonstrated that the performance of GNNs does not always align with homophily metrics, and how homophily influences GNNs still remains unclear and controversial. Then, a crucial question arises: What is missing in our current understanding of homophily? To figure out the missing part, in this paper, we disentangle the graph homophily into $3$ aspects: label, structural, and feature homophily, providing a more comprehensive understanding of GNN performance. To investigate their synergy, we propose a Contextual Stochastic Block Model with $3$ types of Homophily (CSBM-3H), where the topology and feature generation are controlled by the $3$ metrics. Based on the theoretical analysis of CSBM-3H, we derive a new composite metric, named Tri-Hom, that considers all $3$ aspects and overcomes the limitations of conventional homophily metrics. The theoretical conclusions and the effectiveness of Tri-Hom have been verified through synthetic experiments on CSBM-3H. In addition, we conduct experiments on $31$ real-world benchmark datasets and calculate the correlations between homophily metrics and model performance. Tri-Hom has significantly higher correlation values than $17$ existing metrics that only focus on a single homophily aspect, demonstrating its superiority and the importance of homophily synergy. Our code is available at \url{https://github.com/zylMozart/Disentangle_GraphHom}.

==> sections/GraphModelling.tex <==
% Need to review current graph hom papers with questions:
% 1. how to model graph with homophily currently
% 1.2 drawbacks of current graph topology and feature modelling (without neighbor and feature homophily)
% 2. how to model graph topology
% 3. how to model graph feature
For the graph modelling, current studies~\cite{ana_label_info,ana_feat_dist,when_do_graph_help,is_hom_necessary} generally adopt a Contextual Stochastic Block Model(CSBM) to control the label homophily $h_L$ through assigning nodes with the probabilities of the connections to different communities in graphs. Then the node features are independently sampled with respect to their class. However, such way of graph modeling has two drawbacks: First, the neighbor distributions of nodes are fixed, leading to a homogeneous neighbor distribution inside one class. Second, the sampled node features are independent with their neighbors, which is unreasonable in real-world scenarios where interactions change the attributes of connected nodes~\cite{feat_dpd_recm_2,feat_dpd_social_1,feat_dpd_social_2}. Towards a more general and reasonable modelling of graph topology as well as node features, we introduce our modeling of graph topology and node features with the aforementioned homophily definitions, which assumes in a graph, \sitao{Emphasize these assumptions are for simplicity without loss of generality}
\begin{itemize}
    \item all the nodes are class-balanced and have the same degree $d$,
    \item all the classes share the same label homophily $h_L$ and structural homophily $h_S$, and
    \item all the features share a same feature homophily $h_F$.
\end{itemize}

% We first give notations defined in the model. We use $\b{Z}\in \mathbb{R}^{n\times F}$ to denote implicit features and $\b{X}\in \mathbb{R}^{n\times F}$ to denote explicit features. Additionally, we use node labels $\b{Y}\in \mathbb{R}^{n \times C}$ and node degrees $\b{D}\in \mathbb{R}^{n}$ to describe properties of nodes. For the topology, we use $\b{A}\in \mathbb{R}^{n\times n}$ to describe adjacency matrix and $\b{S}\in \mathbb{R}^{C\times C}$ to describe neighbor sampling matrix. For each node $v_i$ belong to class $k$, we assume its implicit features follow a multi-variate Gaussian distribution $\b{z}_i \sim \b{N_k}(\b{\mu}_k,\b{\Sigma}_k)$. Then the implicit features can be described as $\b{Z} = \b{Y}\b{N}$, where$\b{N} = \begin{bmatrix} \b{N_0}, \b{N_1}, \cdots, \b{N_C}\end{bmatrix}^T$.

\subsection{Graph Topology Modelling}

Our graph topology modelling involve both the label homophily $h_L$ and structural homophily $h_S$ that control the consistency of labels across the topology and the consistency of neighbor distributions within each classes. Hence, the neighbor distribution can be represented as:
\begin{equation}
    \mathcal{D}_{\mathcal{N}} = \b{Y}\b{S} 
\end{equation}
where $\b{S}$ is the class-sampling matrix and $\epsilon$ is the observed deviation of each entry of the $\b{S}$ with the variance $\frac{(1-h_S)^2}{c-1}$
\begin{equation}\label{eq:sampling_hl_hs}
\begin{split}
    \b{S} = \begin{bmatrix}
        h_L & \frac{1-h_L}{c-1} & \cdots & \frac{1-h_L}{c-1} \\
        \frac{1-h_L}{c-1} & h_L & \cdots & \frac{1-h_L}{c-1} \\
        \vdots & \vdots & \ddots & \vdots \\
        \frac{1-h_L}{c-1} & \frac{1-h_L}{c-1} & \cdots & h_L \\
    \end{bmatrix} + \b{\epsilon} 
    = \frac{1-h_L}{c-1}\b{1}+(h_L-\frac{1-h_L}{c-1})\b{I}+\b{\epsilon}
\end{split}
\end{equation}
Note that $\mathcal{D}_{\mathcal{N}}$ is a probability matrix with the constraint of $|\mathcal{D}_{{\mathcal{N}},u}|=1$ for all the node $u$. Then, we can get the neighbor-sampling matrix from the neighbor distribution:
\begin{equation}
    \b{A_p} = \frac{cd}{n}\mathcal{D}_{\mathcal{N}}\b{Y}^T
\end{equation}

Finally, we can derive the final adjacency matrix $\b{A}$ by element-wise sampling and symmetrically regularizing $\b{A_p}$:
\begin{equation}
    \b{A} = ( Sym \circ Bernoulli ) (\b{A_p}) 
\end{equation}
\sitao{Such Compound probability distribution makes things complex. See \url{https://en.wikipedia.org/wiki/Compound_probability_distribution}}
where the $bernoulli$ function converts each value into 1 or 0 with given probability and the $Sym$ function turns the non-symmetric matrix to symmetric matrix.

As shown in Eq. (\ref{eq:sampling_hl_hs}), the label homophily $h_L$ controls the ratio of the neighbors that share the same labels as the ego nodes and the structural homophily $h_S$ controls the standard deviation of the neighbor distribution of each class. The $h_L$ and $h_S$ control different aspects of graph, enabling us to study the relation of graph structures with graph models.

\subsection{Graph Feature Modelling}
We first sample the graph features with respect to their classes, which can be expressed as:
\begin{equation}
    \b{X}^0 \sim \b{Y} \b{N}(\b{\mu},\b{\Sigma})
\end{equation}
where $\b{N}(\b{\mu},\b{\Sigma})\in \mathbb{R}^{c\times M}$ is a multi-variate Gaussian distribution and all the variables in $\b{N}$ are independent from each other. 

This kind of feature modelling has been adopted by many studies~\cite{}. However, $\b{X}^0$ only contains the class information while ignoring the dependencies from neighbors, which also constitute an important part of the node features. Hence, we go beyond the feature modelling process from $p(\b{X}|\b{Y})$ to $p(\b{X}|\b{Y},\b{A})$, which considers the dependencies from both the class and topology perspectives. Specifically, we model the dependencies with a first-order temporal dependencies as described in Section \ref{sec:def_h_f}:
\begin{equation}
    \b{X} =\lim_{t\to \infty} \sum_{i=0}^t \left(\frac{h_F}{\sigma(\b{A})}\b{A}\right)^i\b{X}^0 =  \left(\b{I}-\frac{h_F}{\sigma(\b{A})}\b{A}\right)^{-1}\b{X}^0
\end{equation}
where $h_F$ falls into a range of $(-1,1)$, leading to a convergence of $\left(\frac{h_F}{\sigma(\b{A})}\b{A}\right)^i$. This implies the dependencies of node features will fade away as the distances increases. Meanwhile, as shown in \ref{ppt:h_F_sign}, the sign of $h_F$ determines the behavior of the dependencies. When $h_F>0$, the neighboring node features will become more similar while for $h_F<0$, it will be dissimilar. In particular, when $h_F=0$, node features remain independent from each other. This charastistic enables us to investigate the graph behaviors under different scenarios of node dependencies. 

==> tables/correlation_kendall_difference.tex <==
\begin{table}[htbp]
  \centering
  \caption{Kendall’s Tau rank correlation with p-value of all the metrics with the performance differences of GNNs with MLP of node classification on real-world datasets. We measure the correlation and p-value of each homophily metric with model performance on 31 real-world datasets.}
  % \resizebox{1\hsize}{!}{
    \begin{tabular}{lccccccr}
    \toprule
     \multirow{2}{*}{Metric} & \multicolumn{2}{c}{GCN-MLP} & \multicolumn{2}{c}{GraphSage-MLP} & \multicolumn{2}{c}{GAT-MLP} & \multirow{2}{*}{Rank} \\
    \cmidrule{2-7}
    & Cor. & p-value& Cor. & p-value& Cor. & p-value & \\
    \toprule
$h_{edge}$&\textcolor{blue}{0.3462}& 0.0058& 0.2129& 0.0960& 0.2731& 0.0314&\textcolor{purple}{5.83}\\
$h_{node}$&\textcolor{purple}{0.3161}& 0.0122& 0.1828& 0.1545&\textcolor{blue}{0.3118}& 0.0135& 6.33\\
$h_{class}$& 0.1570& 0.2231& 0.1785& 0.1647& 0.2387& 0.0611& 12.83\\
$h_{adj}$& 0.2731& 0.0314& 0.2602& 0.0407& 0.2602& 0.0407& 6.17\\
$h_{den}$& 0.2559& 0.0442& 0.2258& 0.0770& 0.2430& 0.0565& 7.67\\
$h_{2hop}$& 0.1785& 0.1647& 0.1742& 0.1754& 0.0968& 0.4578& 14.83\\
$h_{nei}$& 0.1871& 0.1448& 0.2086& 0.1031& 0.1054& 0.4178& 12.33\\
$LI$&\textcolor{red}{0.3505}& 0.0052& 0.2774& 0.0287&\textcolor{red}{0.3204}& 0.0110&\textcolor{red}{2.67}\\
$h_{NS}$& 0.2473& 0.0521&\textcolor{red}{0.4237}& 0.0006& 0.2258& 0.0770& 6.17\\
$h_{agg}$& 0.0022& 1.0000& 0.2129& 0.0960& 0.0323& 0.8135& 16.83\\
$h_S$& 0.2172& 0.0893& 0.1613& 0.2104&\textcolor{purple}{0.3075}& 0.0149& 10.00\\
$h_{GE}$& 0.1441& 0.2644& 0.2860& 0.0240& 0.0624& 0.6369& 13.33\\
$h_{LS-cos}$& 0.1570& 0.2231& 0.3075& 0.0149& 0.0753& 0.5664& 12.17\\
$h_{LS-euc}$& 0.0409& 0.7616& -0.1527& 0.2363& 0.0968& 0.4578& 18.83\\
$h_{attr}$& -0.2688& 0.0343& -0.4366& 0.0004& -0.2387& 0.0611& 22.00\\
$h_{CF}$& 0.1699& 0.1865&\textcolor{purple}{0.3118}& 0.0135& 0.1742& 0.1754& 9.33\\
$h_F$& 0.3071& 0.0253&\textcolor{blue}{0.4169}& 0.0024& 0.2821& 0.0399&\textcolor{blue}{3.33}\\
$h_{KR}$& 0.2416& 0.0568& 0.0734& 0.5631& 0.2201& 0.0828& 12.67\\
$h_{GNB}$& 0.1093& 0.3935& -0.0874& 0.4948& 0.1487& 0.2458& 17.00\\
$h_{SVM}$& -0.1753& 0.1752& -0.0067& 0.9589& -0.0688& 0.5948& 20.33\\
$\mathcal{J}^{\neg\mathcal{G}}$& 0.1369& 0.3108& 0.2004& 0.1378& 0.1027& 0.4472& 15.00\\
$\mathcal{J}^{\mathcal{G}}$& 0.2473& 0.0521& 0.2344& 0.0661& 0.2602& 0.0407& 7.33\\
    \bottomrule
    \end{tabular}%
% }
  \label{tab:kendall_acc_diff}%
\end{table}%

==> tables/correlation_kendall_model.tex <==
\begin{table}[htbp]
  \centering
  \caption{Kendall’s Tau rank correlation with p-value of all the metrics with model performance of node classification on real-world datasets. We measure the correlation and p-value of each homophily metric with model performance on 31 real-world datasets.}
  \resizebox{1\hsize}{!}{
    \begin{tabular}{lccccccccr}
    \toprule
     \multirow{2}{*}{Metric} & \multicolumn{2}{c}{MLP} & \multicolumn{2}{c}{GCN} & \multicolumn{2}{c}{GraphSage} & \multicolumn{2}{c}{GAT} & \multirow{2}{*}{Rank} \\
    \cmidrule{2-9}
    & Cor. & p-value& Cor. & p-value& Cor. & p-value& Cor. & p-value & \\
    \toprule
$h_{edge}$& 0.3677& 0.0033&\textcolor{blue}{0.4882}& 0.0001& 0.4452& 0.0003&\textcolor{purple}{0.4839}& 0.0001&\textcolor{purple}{4.12}\\
$h_{node}$& 0.3204& 0.0110& 0.4409& 0.0004& 0.4065& 0.0011& 0.4624& 0.0002& 8.75\\
$h_{class}$&\textcolor{blue}{0.3935}& 0.0016& 0.4194& 0.0007& 0.4022& 0.0012& 0.4237& 0.0006& 7.25\\
$h_{adj}$&\textcolor{purple}{0.3892}& 0.0018& 0.4667& 0.0001& 0.4323& 0.0005& 0.4538& 0.0002& 5.62\\
$h_{den}$& 0.2430& 0.0565& 0.3634& 0.0037& 0.3548& 0.0047& 0.3677& 0.0033& 13.25\\
$h_{2hop}$&\textcolor{purple}{0.3892}& 0.0018& 0.4065& 0.0011& 0.3720& 0.0029& 0.3935& 0.0016& 8.62\\
$h_{nei}$& 0.3376& 0.0073& 0.3720& 0.0029& 0.3462& 0.0058& 0.3591& 0.0042& 12.38\\
$LI$& 0.3462& 0.0058&\textcolor{purple}{0.4753}& 0.0001& 0.4409& 0.0004&\textcolor{blue}{0.5054}& 0.0000& 4.88\\
$h_{NS}$& 0.3720& 0.0029& 0.4581& 0.0002& 0.4409& 0.0004& 0.4710& 0.0001& 5.62\\
$h_{agg}$& 0.3849& 0.0020& 0.4452& 0.0003&\textcolor{blue}{0.4624}& 0.0002& 0.4495& 0.0003& 5.50\\
$h_S$& 0.0667& 0.6130& 0.2387& 0.0611& 0.2129& 0.0960& 0.2774& 0.0287& 17.25\\
$h_{GE}$& 0.3376& 0.0073& 0.3376& 0.0073& 0.3290& 0.0090& 0.3247& 0.0100& 13.88\\
$h_{LS-cos}$& 0.3677& 0.0033& 0.3591& 0.0042& 0.3505& 0.0052& 0.3462& 0.0058& 12.12\\
$h_{LS-euc}$& -0.2989& 0.0181& -0.2387& 0.0611& -0.2559& 0.0442& -0.2172& 0.0893& 19.75\\
$h_{attr}$& -0.1183& 0.3617& -0.2903& 0.0218& -0.2817& 0.0263& -0.2688& 0.0343& 20.50\\
$h_{CF}$& 0.2860& 0.0240& 0.2946& 0.0199& 0.3032& 0.0164& 0.3075& 0.0149& 15.75\\
$h_F$& 0.2871& 0.0365& 0.3920& 0.0043& 0.3870& 0.0048& 0.3920& 0.0043& 11.50\\
$h_{KR}$& -0.4186& 0.0010& -0.3236& 0.0107& -0.3495& 0.0059& -0.3279& 0.0097& 22.00\\
$h_{GNB}$& -0.2929& 0.0222& -0.2317& 0.0704& -0.2580& 0.0440& -0.2361& 0.0653& 19.75\\
$h_{SVM}$& 0.1531& 0.2364& 0.1176& 0.3631& 0.1398& 0.2797& 0.1309& 0.3114& 17.75\\
$\mathcal{J}^{\neg\mathcal{G}}$&\textcolor{red}{0.4106}& 0.0024& 0.4693& 0.0005&\textcolor{purple}{0.4546}& 0.0008& 0.4790& 0.0004&\textcolor{red}{3.00}\\
$\mathcal{J}^{\mathcal{G}}$& 0.3290& 0.0090&\textcolor{red}{0.5097}& 0.0000&\textcolor{red}{0.4753}& 0.0001&\textcolor{red}{0.5398}& 0.0000&\textcolor{blue}{3.75}\\
    \bottomrule
    \end{tabular}%
}
  \label{tab:kendall_acc_model}%
\end{table}%

==> tables/correlation_spearman.tex <==
\begin{table}[htbp]
  \centering
  \caption{Spearman rank correlation of all the metrics with model performance of node classification on real-world datasets}
  \resizebox{1\hsize}{!}{
    \begin{tabular}{lcccccccccccccc}
    \toprule
     \multirow{2}{*}{Metric} & \multicolumn{2}{c}{MLP} & \multicolumn{2}{c}{GCN} & \multicolumn{2}{c}{GraphSage} & \multicolumn{2}{c}{GAT} & \multicolumn{2}{c}{GCN-MLP} & \multicolumn{2}{c}{GraphSage-MLP} & \multicolumn{2}{c}{GAT-MLP}\\
    \cmidrule{2-15}
    & \multicolumn{2}{c}{Cor.\ /\ p-value}& \multicolumn{2}{c}{Cor.\ /\ p-value}& \multicolumn{2}{c}{Cor.\ /\ p-value}& \multicolumn{2}{c}{Cor.\ /\ p-value} & \multicolumn{2}{c}{Cor.\ /\ p-value}& \multicolumn{2}{c}{Cor.\ /\ p-value}& \multicolumn{2}{c}{Cor.\ /\ p-value} \\
    \toprule
$h_{edge}$& 0.4560 & 0.0099& 0.6137 & 0.0002& 0.5552 & 0.0012& 0.6004 & 0.0004&\underline{0.4266}& 0.0167& 0.2911 & 0.1121& 0.3552 & 0.0499\\
$h_{node}$& 0.4121 & 0.0212& 0.5569 & 0.0011& 0.4956 & 0.0046& 0.5681 & 0.0009& 0.3968 & 0.0271& 0.2468 & 0.1808& 0.4109 & 0.0217\\
$h_{class}$& 0.5246 & 0.0024& 0.5351 & 0.0019& 0.4980 & 0.0044& 0.5512 & 0.0013& 0.2375 & 0.1983& 0.2278 & 0.2177& 0.3145 & 0.0848\\
$h_{adj}$& 0.4927 & 0.0049& 0.5766 & 0.0007& 0.5347 & 0.0019& 0.5661 & 0.0009& 0.3452 & 0.0572& 0.3190 & 0.0803& 0.3290 & 0.0707\\
$h_{den}$& 0.3823 & 0.0338& 0.5423 & 0.0016& 0.5125 & 0.0032& 0.5399 & 0.0017& 0.3625 & 0.0451& 0.3266 & 0.0729& 0.3649 & 0.0435\\
$h_{2hop}$& 0.4855 & 0.0056& 0.5266 & 0.0023& 0.4891 & 0.0052& 0.5032 & 0.0039& 0.2444 & 0.1852& 0.2028 & 0.2738& 0.1266 & 0.4973\\
$h_{nei}$& 0.4242 & 0.0174& 0.4754 & 0.0069& 0.4395 & 0.0134& 0.4516 & 0.0108& 0.2613 & 0.1557& 0.2435 & 0.1867& 0.1375 & 0.4607\\
$LI$& 0.4452 & 0.0121&\underline{0.6403}& 0.0001& 0.5899 & 0.0005& 0.6419 & 0.0001& 0.4177 & 0.0194& 0.3355 & 0.0650& 0.3891 & 0.0305\\
$h_{NS}$& 0.5137 & 0.0031&\textbf{0.6419}& 0.0001&\underline{0.6335}& 0.0001&\underline{0.6456}& 0.0001& 0.3327 & 0.0675&\textbf{0.6008}& 0.0004& 0.3302 & 0.0696\\
$h_{agg}$&\underline{0.5343}& 0.0020& 0.6246 & 0.0002&\textbf{0.6520}& 0.0001& 0.6367 & 0.0001& 0.0258 & 0.8904& 0.3569 & 0.0488& 0.1028 & 0.5820\\
$h_S$& 0.1536 & 0.4093& 0.3758 & 0.0372& 0.3440 & 0.0581& 0.4230 & 0.0177& 0.3141 & 0.0853& 0.2210 & 0.2323&\textbf{0.4403}& 0.0132\\
$h_{GE}$& 0.4665 & 0.0082& 0.4762 & 0.0068& 0.4681 & 0.0079& 0.4565 & 0.0098& 0.2161 & 0.2429& 0.3327 & 0.0675& 0.0851 & 0.6491\\
$h_{LS-cos}$& 0.4839 & 0.0058& 0.4855 & 0.0056& 0.4754 & 0.0069& 0.4661 & 0.0082& 0.2339 & 0.2054& 0.3589 & 0.0474& 0.1073 & 0.5658\\
$h_{LS-euc}$& -0.4407 & 0.0131& -0.3472 & 0.0557& -0.3512 & 0.0527& -0.3222 & 0.0771& 0.0427 & 0.8194& -0.1282 & 0.4918& 0.1165 & 0.5324\\
$h_{attr}$& -0.1452 & 0.4359& -0.3669 & 0.0423& -0.3657 & 0.0430& -0.3520 & 0.0521& -0.4113 & 0.0215& -0.6266 & 0.0002& -0.3375 & 0.0633\\
$h_{CF}$& 0.3649 & 0.0435& 0.4202 & 0.0186& 0.4181 & 0.0192& 0.4222 & 0.0180& 0.2306 & 0.2119& 0.4302 & 0.0157& 0.2165 & 0.2420\\
$h_F$& 0.3718 & 0.0394& 0.5296 & 0.0022& 0.5147 & 0.0030& 0.5296 & 0.0022&\textbf{0.4309}& 0.0155&\underline{0.5831}& 0.0006& 0.3944 & 0.0281\\
$h_{KR1}$& -0.5970 & 0.0004& -0.4187 & 0.0191& -0.4550 & 0.0101& -0.4223 & 0.0179& 0.3546 & 0.0503& 0.0932 & 0.6181& 0.3159 & 0.0835\\
$h_{GNB}$& -0.4512 & 0.0108& -0.3723 & 0.0392& -0.3933 & 0.0286& -0.3527 & 0.0517& 0.1441 & 0.4394& -0.0872 & 0.6409& 0.2050 & 0.2687\\
$h_{SVM}$& 0.2021 & 0.2755& 0.1633 & 0.3801& 0.2040 & 0.2711& 0.2021 & 0.2755& -0.2481 & 0.1784& -0.0352 & 0.8510& -0.1171 & 0.5303\\
$\mathcal{J}^{\neg\mathcal{G}}$&\textbf{0.5399}& 0.0017& 0.6340 & 0.0001& 0.6092 & 0.0003& 0.6285 & 0.0002& 0.1978 & 0.2862& 0.2967 & 0.1051& 0.1623 & 0.3832\\
$\mathcal{J}^{\mathcal{G}}$& 0.4794 & 0.0064& 0.6294 & 0.0001& 0.5851 & 0.0005&\textbf{0.6516}& 0.0001& 0.3915 & 0.0294& 0.3145 & 0.0848&\underline{0.4294}& 0.0159\\
    \bottomrule
    \end{tabular}%
}
  \label{tab:cor_spearman}%
\end{table}%

==> tables/hom_acc_correlation.tex <==
\begin{table}[htbp]
  \centering
  \caption{Pearson correlation of all the metrics with model performance of node classification on real-world datasets. We measure the correlation and p-value of each homophily metric with model performance on 31 real-world datasets.}
  \resizebox{1\hsize}{!}{
    \begin{tabular}{lcccccccccccccc}
    \toprule
     \multirow{2}{*}{Metric} & \multicolumn{2}{c}{MLP} & \multicolumn{2}{c}{GCN} & \multicolumn{2}{c}{GraphSage} & \multicolumn{2}{c}{GAT} & \multicolumn{2}{c}{GCN-MLP} & \multicolumn{2}{c}{GraphSage-MLP} & \multicolumn{2}{c}{GAT-MLP}\\
    \cmidrule{2-15}
    & \multicolumn{2}{c}{Cor.\ /\ p-value}& \multicolumn{2}{c}{Cor.\ /\ p-value}& \multicolumn{2}{c}{Cor.\ /\ p-value}& \multicolumn{2}{c}{Cor.\ /\ p-value} & \multicolumn{2}{c}{Cor.\ /\ p-value}& \multicolumn{2}{c}{Cor.\ /\ p-value}& \multicolumn{2}{c}{Cor.\ /\ p-value} \\
    \toprule
$h_{edge}$& 0.4441 & 0.0123& 0.5663 & 0.0009& 0.4737 & 0.0071& 0.5344 & 0.0020& 0.2937 & 0.1087& 0.1189 & 0.5242& 0.2073 & 0.2632\\
$h_{node}$& 0.4232 & 0.0177& 0.5457 & 0.0015& 0.4524 & 0.0106& 0.5257 & 0.0024& 0.2930 & 0.1097& 0.1155 & 0.5362& 0.2316 & 0.2099\\
$h_{class}$&\textcolor{red}{0.6078}& 0.0003&\textcolor{purple}{0.6120}& 0.0003& 0.5790 & 0.0006&\textcolor{blue}{0.6169}& 0.0002& 0.0454 & 0.8084& 0.0075 & 0.9678& 0.0459 & 0.8064\\
$h_{adj}$& 0.4972 & 0.0044& 0.5486 & 0.0014& 0.4932 & 0.0048& 0.5396 & 0.0017& 0.1420 & 0.4461& 0.0500 & 0.7896& 0.1101 & 0.5555\\
$h_{den}$& 0.0038 & 0.9839& 0.1483 & 0.4258& 0.0525 & 0.7791& 0.1258 & 0.5001&\textcolor{blue}{0.3164}& 0.0829& 0.1096 & 0.5572& 0.2537 & 0.1685\\
$h_{2hop}$& 0.4517 & 0.0107& 0.5182 & 0.0028& 0.4692 & 0.0078& 0.4870 & 0.0055& 0.1722 & 0.3543& 0.0925 & 0.6208& 0.0932 & 0.6178\\
$h_{nei}$& 0.3961 & 0.0274& 0.4793 & 0.0064& 0.4473 & 0.0116& 0.4535 & 0.0104& 0.2055 & 0.2675& 0.1615 & 0.3854& 0.1367 & 0.4632\\
$LI$& 0.4502 & 0.0110& 0.4992 & 0.0043& 0.4270 & 0.0166& 0.4731 & 0.0072& 0.1338 & 0.4729& 0.0012 & 0.9948& 0.0674 & 0.7186\\
$h_{NS}$& 0.2898 & 0.1139& 0.3603 & 0.0465& 0.3452 & 0.0572& 0.3671 & 0.0422& 0.1716 & 0.3561& 0.1585 & 0.3945& 0.1736 & 0.3503\\
$h_{agg}$& 0.5201 & 0.0027& 0.5617 & 0.0010&\textcolor{blue}{0.6040}& 0.0003& 0.5832 & 0.0006& 0.1220 & 0.5132&\textcolor{blue}{0.2497}& 0.1755& 0.1542 & 0.4076\\
$h_S$& 0.0981 & 0.5994& 0.2345 & 0.2042& 0.1981 & 0.2854& 0.2886 & 0.1153&\textcolor{purple}{0.3040}& 0.0964&\textcolor{purple}{0.2356}& 0.2020&\textcolor{red}{0.4001}& 0.0257\\
$h_{GE}$& 0.3641 & 0.0440& 0.4501 & 0.0111& 0.4347 & 0.0145& 0.4094 & 0.0222& 0.2096 & 0.2577& 0.2011 & 0.2779& 0.1102 & 0.5550\\
$h_{LS-cos}$& 0.3511 & 0.0528& 0.4389 & 0.0135& 0.4254 & 0.0170& 0.4061 & 0.0234& 0.2130 & 0.2500& 0.2080 & 0.2614& 0.1299 & 0.4862\\
$h_{LS-euc}$& 0.1272 & 0.4953& 0.1101 & 0.5555& 0.1117 & 0.5498& 0.1168 & 0.5313& -0.0299 & 0.8733& -0.0197 & 0.9160& -0.0159 & 0.9323\\
$h_{attr}$& 0.2022 & 0.2754& 0.0990 & 0.5963& 0.0735 & 0.6945& 0.1121 & 0.5482& -0.2137 & 0.2484& -0.2644 & 0.1506& -0.1781 & 0.3376\\
$h_{CF}$& 0.2549 & 0.1664& 0.2890 & 0.1149& 0.3154 & 0.0840& 0.3167 & 0.0825& 0.0897 & 0.6313& 0.1657 & 0.3730& 0.1398 & 0.4531\\
$h_F$& 0.4035 & 0.0244& 0.4994 & 0.0042& 0.4814 & 0.0061& 0.4767 & 0.0067& 0.2338 & 0.2056& 0.2224 & 0.2292& 0.1701 & 0.3604\\
$h_{KR}$& -0.5318 & 0.0021& -0.3536 & 0.0510& -0.3854 & 0.0323& -0.3599 & 0.0468&\textcolor{red}{0.3582}& 0.0478&\textcolor{red}{0.2650}& 0.1497&\textcolor{blue}{0.3336}& 0.0667\\
$h_{GNB}$& -0.3796 & 0.0352& -0.2440 & 0.1858& -0.2828 & 0.1232& -0.2421 & 0.1894& 0.2740 & 0.1357& 0.1721 & 0.3546& 0.2689 & 0.1435\\
$h_{SVM}$& 0.2430 & 0.1878& 0.2741 & 0.1356& 0.3320 & 0.0681& 0.2961 & 0.1058& 0.0825 & 0.6590& 0.2281 & 0.2171& 0.1211 & 0.5162\\
$\mathcal{J}^{\neg\mathcal{G}}$&\textcolor{blue}{0.5800}& 0.0006&\textcolor{blue}{0.6286}& 0.0002&\textcolor{purple}{0.5978}& 0.0004&\textcolor{purple}{0.6136}& 0.0002& 0.1407 & 0.4503& 0.1086 & 0.5610& 0.0954 & 0.6096\\
$\mathcal{J}^{\mathcal{G}}$&\textcolor{purple}{0.5471}& 0.0014&\textcolor{red}{0.6650}& 0.0000&\textcolor{red}{0.6223}& 0.0002&\textcolor{red}{0.6731}& 0.0000& 0.2903 & 0.1131& 0.2333 & 0.2065&\textcolor{purple}{0.2860}& 0.1188\\
    \bottomrule
    \end{tabular}%
}
  \label{tab:hom_acc_cor}%
\end{table}%
